Particle MPC for Uncertain and Learning-Based Control

As robotic systems move from highly structured environments to open worlds, incorporating uncertainty from dynamics learning or state estimation into the control pipeline is essential for robust performance. In this paper we present a nonlinear particle model predictive control (PMPC) approach to control under uncertainty, which directly incorporates any particle-based uncertainty representation, such as those common in robotics. Our approach builds on scenario methods for MPC, but in contrast to existing approaches, which either constrain all or only the first timestep to share actions across scenarios, we investigate the impact of a \textit{partial consensus horizon}. Implementing this optimization for nonlinear dynamics by leveraging sequential convex optimization, our approach yields an efficient framework that can be tuned to the particular information gain dynamics of a system to mitigate both over-conservatism and over-optimism. We investigate our approach for two robotic systems across three problem settings: time-varying, partially observed dynamics; sensing uncertainty; and model-based reinforcement learning, and show that our approach improves performance over baselines in all settings.

==> notation.tex <==
\begin{table}[H]
\centering
\begin{tabular}{p{0.45\linewidth}  p{0.55\linewidth}}
$i, M$ & particle index, particle number\\
$j, N$ & time step index, horizon length\\
$N_c$ & consensus horizon\\
\\
$x^{(j)} \in \mathbb{R}^s, u^{(j)} \in \mathbb{R}^a$ & state and control vectors\\
\\
$\widehat{x}^{(j)}, \widehat{u}^{(j)}$ & a linearization point\\
$f^{(j)} = f(\widehat{x}^{(j)}, \widehat{u}^{(j)})$ & dynamics transition\\
$f^{(j)}_x = f_x(\widehat{x}^{(j)}, \widehat{u}^{(j)}) \in \mathbb{R}^{s \times s}$ &
dynamics state Jacobian\\
$f^{(j)}_u = f_u(\widehat{x}^{(j)}, \widehat{u}^{(j)}) \in \mathbb{R}^{s \times a}$ &
dynamics control Jacobian\\ 
\\
$x_{ref}^{(j)}, u_{ref}^{(j)}$ & reference trajectory\\
$Q^{(j)}, R^{(j)}$ & state and control quadratic cost\\
\\
$x \in \mathbb{R}^{N s}, u \in \mathbb{R}^{N a}$ & trajectory variables \\
$v = (x, u) \in \mathbb{R}^{N (s + a)}$ & concatenated trajectory variables \\
$A \in \mathbb{R}^{N s \times N (s + a)}$ & dynamics feasibility matrix\\
$b \in \mathbb{R}^{N s} $ & dynamics feasibility vector \\
$P \in \mathbb{R}^{N (s + a) \times N (s + a)}$ & quadratic cost matrix \\
$q \in \mathbb{R}^{N (s + a)}$ & quadratic sot vector \\
$b_l \in \mathbb{R}^{N (s + a)}$ & state and control lower box bound\\
$b_u \in \mathbb{R}^{N (s + a)}$ & state and control upper box bound\\
$c_i(x, u)$ & cost for the $i$-th particle\\
$c(x^{(j)}, u^{(j)})$ & cost at the $j$-th time step\\
\\
$\mathcal{X}_0$ & initial state uncertainty distribution \\
$\mathcal{F}, \mathcal{F}_x, \mathcal{F}_u$ & dynamics uncertainty distribution \\
$\mathcal{W}_0$ & additive noise distribution \\
\end{tabular}
\end{table}


==> results.tex <==
\section{Tabulated Results}

% ---------------------------------------------------------------------------- %
\subsection{Model uncertainty}

\subsubsection{Freeflier}
\subsubsection{Planar quadrotor}

% ---------------------------------------------------------------------------- %
\subsection{Sensing uncertainty}

\subsubsection{Freeflier}
\subsubsection{Planar quadrotor}

% ---------------------------------------------------------------------------- %
\subsection{Learning for control}

\subsubsection{Freeflier}
\subsubsection{Planar quadrotor}

Total collisions in training

\begin{table}
\begin{tabular}{c c}
\toprule
{Method} & {Total collisions in trainig} \\
\midrule
{PMPC, $Nc = 1$} & $5.8 \pm 0.6$ \\
{PMPC, $Nc = 5$} & $4.4 \pm 0.4$ \\
{PMPC, $Nc = 10$} & $\bm{3.7} \pm 0.2$ \\
{CE} & $5.7 \pm 0.3$ \\
\bottomrule
\end{tabular}
\caption{Learning}
\end{table}

